Exploiting Code Symmetries for Learning Program Semantics

This paper tackles the challenge of teaching code semantics to Large Language Models (LLMs) for program analysis by incorporating code symmetries into the model architecture. We introduce a group-theoretic framework that defines code symmetries as semantics-preserving transformations, where forming a code symmetry group enables precise and efficient reasoning of code semantics. Our solution, SymC, develops a novel variant of self-attention that is provably equivariant to code symmetries from the permutation group defined over the program dependence graph. SymC obtains superior performance on five program analysis tasks, outperforming state-of-the-art code models without any pre-training. Our results suggest that code LLMs that encode the code structural prior via the code symmetry group generalize better and faster.

==> motivate.tex <==
\section{Motivating Example}
\label{sec:motivating_example}

% Before formally defining semantics-preserving symmetries and their significance in generalizability, we present an intuitive example to illustrate our symmetry-preserving construction. 
Figure~\ref{subfig:example-g-invariant} depicts an ideal code model for vulnerability detection, with the representation learning $r$ and predictive learning $p$ components.
% Specifically, its representation learning $r$ stays equivariant and predictive learning $p$ stays invariant to the permutations of input statements. 
% Figure~\ref{subfig:example-g-invariant} demonstrates a vulnerability predictor ($p\circ r$) satisfying $G$-invariance with respect to a permutation group $G$. 
The code snippets with an integer overflow vulnerability illustrate a semantics-preserving statement reordering. 
Such permutations should not change the final prediction (\ie vulnerable), as $c_1$ has no data/control dependency with the other lines. 
This intuition is enforced through $G$-invariance, ensuring the final vulnerability prediction remains unchanged (\ie vulnerable), and $G$-equivariance, where the code representation $(e_1,...,e_4)$ is transformed into $(e_2,...,e_4, e_1)$, preserving equivariance to the permutations in $G$.

\begin{wrapfigure}[18]{r}{.75\textwidth}

    \begin{center}
    \vspace{-2em}
    
    % \subfloat[$G$-invariant code analysis]{
    % \includegraphics[width=0.19\linewidth]{./figs/motivate/equivariant-invariant1.pdf}
    % \label{subfig:abstract-g-invariant}}\hspace{-.4cm}%
    \subfloat[$G$-invariant vulnerability detector]{
    \includegraphics[width=0.49\linewidth]{./figs/motivate/equivariant-invariant2.pdf}
    \label{subfig:example-g-invariant}}\hspace{-.3cm}%
    \subfloat[Existing vulnerability detector]{
    \includegraphics[width=0.5\linewidth]{./figs/motivate/equivariant-invariant3.pdf}
    \label{subfig:example-g-variant}}

    \caption{
    % (a) High-level summary of $G$-equivariant code representation learning (Definition~\ref{def:g-equivariant-r}) and $G$-invariant predictive learning (Definition~\ref{def:g-invariant-p}). 
    (a) An $G$-invariant vulnerability detector where $G$ is a group of semantics-preserving statement permutations $g$.
    (b) A vulnerability predictor that does not preserve the symmetries in $G$, \ie the learned statement representation completely changes when they are permuted, and thus incorrectly predicts a vulnerable code as benign.}
    \label{fig:motivating-example}
    \end{center}
\end{wrapfigure}

By contrast, Figure~\ref{subfig:example-g-variant} shows an existing code model (\eg based on Transformer~\citep{pei2020trex}) that does not preserve permutation symmetry. 
In this case, the code representation $(e_1,...,e_4)$ is transformed into a different set of embeddings $(e'_1,...,e'_4)$. 
Consequently, such a representation leads to incorrectly predicting the code snippet to be benign.

%It is important to note that the code snippet in Figure~\ref{fig:equivariant-invariant} cannot be arbitrarily permuted without changing the code semantics (i.e., input-output behavior) since $c_2$, $c_3$, and $c_4$ have dependencies. Thus, the code analysis model $p\circ r$ should not remain invariant to arbitrary permutations, meaning that $G$ is not a simple permutation group. In \S\ref{sec:method}, we will provide a formalization of semantics-preserving symmetries of code and the desired properties for the symmetry group $G$ against which a code analysis model should ideally be invariant.

==> permute.tex <==
\begin{algorithm}
\caption{
% Generating symmetry-preserving Permutations of a Program Dependency graph for Evaluation.
Automorphism sampling.
}

\label{alg:topological_permutation}

\begin{algorithmic}[1]
\Procedure{TopologicalSort}{$G$} \Comment{$G$ is the input directed graph}
\State $\text{visited} \gets \{\text{false}\}$ \Comment{Array to track visited vertices}
\State $\text{stack} \gets \{\}$ \Comment{Stack to store the topological order}

\ForAll{vertices $v$ in $G$}
    \If{$\text{visited}[v] = \text{false}$}
        \State \Call{DFS}{$v, G, \text{visited}, \text{stack}$}
    \EndIf
\EndFor

\State \textbf{output} $\text{stack}$ \Comment{Print the topological order}
\EndProcedure

\Procedure{DFS}{$v, G, \text{visited}, \text{stack}$}
\State $\text{visited}[v] \gets \text{true}$ \Comment{Mark $v$ as visited}

\ForAll{adjacent vertices $u$ of $v$ in $G$}
    \If{$\text{visited}[u] = \text{false}$}
        \State \Call{DFS}{$u, G, \text{visited}, \text{stack}$}
    \EndIf
\EndFor

\State $\text{stack}.\text{push}(v)$ \Comment{Push $v$ onto the stack}
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> tables/dataset.tex <==
\begin{table}[!t]
\small
\setlength{\tabcolsep}{10pt}
\centering
\renewcommand{\arraystretch}{1.1}
% \setlength\aboverulesep{0.4pt}
% \setlength\belowrulesep{0.4pt}

\caption{The statistics of our dataset. For binary code, the datasets are categorized by compilers, optimizations, obfuscations, and lengths. For source code, we follow the categorization from the original paper providing them.}
% \begin{tabular}{l|r||l|r||l|r}
% \toprule[1.1pt]
% \textbf{Project} & \textbf{\# Bins} & \textbf{Project} & \textbf{\# Bins} & \textbf{Project} & \textbf{\# Bins} \\
% \midrule[.9pt]
% bash & 24 & findutils & 78 & nano & 22 \\
% bc & 52 & gawk & 224 & openssl & 24\\
% binutils & 368 & grep & 26 & putty & 125\\
% bison & 26 & gtypist & 22 & sed & 16\\
% busybox & 16 & gzip & 26 & sg3\_utils & 1136\\
% cflow & 26 & ImageMagick & 52 & sqlite & 32\\
% coreutils & 2816 & indent & 16 & usbutils & 44 \\
% curl & 32 & inetutils & 246 & wget & 12\\
% diffutils & 96 & less & 66 & wget2 & 312\\
% \bottomrule[1.1pt]
% \end{tabular}

\begin{tabular}{lrrr}
\toprule
 & \textbf{\# Files} & \textbf{\# Funcs}  & \textbf{\# Insts} \\
\midrule
\multicolumn{4}{l}{\bf Binary: Compiler\vspace{.1cm}}  \\
\texttt{GCC} & 1,140 & 274,840 & 33,464,420    \\
\texttt{Clang} & 1,136 & 279,832 & 31,949,673    \\ \midrule
\multicolumn{4}{l}{\bf Binary: Optimization\vspace{.1cm}}   \\
\texttt{O0} & 285 & 98,451 & 10,202,328    \\
\texttt{O1} & 285 & 61,298 & 7,096,903   \\
\texttt{O2} & 285 & 61,298 & 7,096,903   \\
\texttt{O3} & 285 & 57,023 & 9,101,578   \\ \midrule
\multicolumn{4}{l}{\bf Binary: Obfuscation\vspace{.1cm}}   \\
\texttt{bcf} & 158 & 61,701 & 9,173,168    \\
\texttt{cff} & 158 & 59,724 & 11,146,990    \\
\texttt{ind} & 158 & 56,291 & 2,501,422   \\
\texttt{spl} & 158 & 61,379 & 9,652,268   \\
\texttt{sub} & 158 & 59,694 & 6,198,900   \\ \midrule
% \multicolumn{4}{l}{\bf Binary: Length\vspace{.1cm}}  \\
% \texttt{[7-10]} &  & &    \\
% \texttt{[11-20]} &  & &    \\
% \texttt{[21-50]} &  & &   \\
% \texttt{[51-]} &  & &   \\ \midrule
\multicolumn{4}{l}{\bf Source: Java\vspace{.1cm}}   \\
Java-Small &  & &    \\
Java-Med &  & &    \\
Java-Large &  & &   \\ \midrule
\multicolumn{4}{l}{\bf Source: Python\vspace{.1cm}}   \\
CodeXGLUE &  & &    \\ 
CodeContest &  & &    \\ \bottomrule
\end{tabular}

\label{tab:datasets}
\end{table}
